Exploiting auto-encoders and segmentation methods for middle-level explanations of image classification systems

A central issue addressed by the rapidly growing research area of eXplainable Artificial Intelligence (XAI) is to provide methods to give explanations for the behaviours of Machine Learning (ML) non-interpretable models after the training. Recently, it is becoming more and more evident that new directions to create better explanations should take into account what a good explanation is to a human user. This paper suggests taking advantage of developing an XAI framework that allows producing multiple explanations for the response of image a classification system in terms of potentially different middle-level input features. To this end, we propose an XAI framework able to construct explanations in terms of input features extracted by auto-encoders. We start from the hypothesis that some autoencoders, relying on standard data representation approaches, could extract more salient and understandable input properties, which we call here \textit{Middle-Level input Features} (MLFs), for a user with respect to raw low-level features. Furthermore, extracting different types of MLFs through different type of autoencoders, different types of explanations for the same ML system behaviour can be returned. We experimentally tested our method on two different image datasets and using three different types of MLFs. The results are encouraging. Although our novel approach was tested in the context of image classification, it can potentially be used on other data types to the extent that auto-encoders to extract humanly understandable representations can be applied.

==> __tables.tex <==
\begin{table}[ht!]\centering
\color{red}
\caption{\color{red} average AOPC of the proposed methods and LIME obtained averaging over the last AOPC perturbation step on a sample of $100$ random images taken from STL10 dataset. Flat and hierarchical proposal are compared with LIME, resulting better in both cases. Since the LIME MLFs structure is hardly different from VAE MLFs (the former corresponds to superpixels, the latter to latent variables), the AOPC reported has not to be compared with the other results.}\label{tab:aopc_stl10}
\scriptsize
\begin{tabular}{lrr}\toprule
\textbf{} &\textbf{AOPC} \\\midrule
LIME &0.042 \\
Flat (proposed) &0.598 \\
Hierarchical (proposed) &\textbf{0.732} \\
\hdashline 
VAE (proposed) &0.595 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!htp]\centering
\color{red}
\caption{\color{red} average AOPC  of the proposed methods and LIME obtained averaging over the last AOPC perturbation step values on a sample of $50$ random images taken from Aberdeen dataset.}\label{tab:aopc_aberdeen}
\scriptsize
\begin{tabular}{lrr}\toprule
\textbf{} &\textbf{AOPC} \\\midrule
LIME &0.014 \\
Flat (proposed) &0.571 \\
Hierarchical (proposed) &\textbf{0.661} \\
\bottomrule
\end{tabular}
\end{table}
